Synthesizing Modular Invariants for Synchronous Code

In this paper, we explore different techniques to synthesize modular invariants for synchronous code encoded as Horn clauses. Modular invariants are a set of formulas that characterizes the validity of predicates. They are very useful for different aspects of analysis, synthesis, testing and program transformation. We describe two techniques to generate modular invariants for code written in the synchronous dataflow language Lustre. The first technique directly encodes the synchronous code in a modular fashion. While in the second technique, we synthesize modular invariants starting from a monolithic invariant. Both techniques, take advantage of analysis techniques based on property-directed reachability. We also describe a technique to minimize the synthesized invariants.

==> eptcsdata.tex <==
\providecommand{\firstpage}{19}
\providecommand{\publicationstatus}{Nikolaj Bj{\o}rner, Fabio Fioravanti, Andrey Rybalchenko, \\ Valerio Senni (Eds.): First Workshop on \\ Horn Clauses for Verification and Synthesis (HCVS 2014)\\
EPTCS 169, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.169.4}{10.4204/EPTCS.169.4}}
\pdfoutput=1

